Short-and-Sparse Deconvolution -- A Geometric Approach

Short-and-sparse deconvolution (SaSD) is the problem of extracting localized, recurring motifs in signals with spatial or temporal structure. Variants of this problem arise in applications such as image deblurring, microscopy, neural spike sorting, and more. The problem is challenging in both theory and practice, as natural optimization formulations are nonconvex. Moreover, practical deconvolution problems involve smooth motifs (kernels) whose spectra decay rapidly, resulting in poor conditioning and numerical challenges. This paper is motivated by recent theoretical advances, which characterize the optimization landscape of a particular nonconvex formulation of SaSD. This is used to derive a $provable$ algorithm which exactly solves certain non-practical instances of the SaSD problem. We leverage the key ideas from this theory (sphere constraints, data-driven initialization) to develop a $practical$ algorithm, which performs well on data arising from a range of application areas. We highlight key additional challenges posed by the ill-conditioning of real SaSD problems, and suggest heuristics (acceleration, continuation, reweighting) to mitigate them. Experiments demonstrate both the performance and generality of the proposed method.

==> sec/exp_img_deblur.tex <==

%Image deblurring aims to recover a sharp
%natural image from its blurred observation due to some unknown photographic process,
%such as a shaking camera or defocusing [28–30]. Although natural images are generally not
%sparse, it is widely acknowledged that sparsity exists in its spatial gradient [28, 31].

==> sec/exp_spikesorting.tex <==

Spike sorting is a crucial first step in extracting neural signals from large-scale electrophysiological data. Usually, electrodes will simultaneously record spike trains from multiple neurons \cite{rey2015past}.The goal of spike sorting is to detect all the spiking times from the measurement and assign detected spikes to specific neurons. We refer interested readers to \cite{lewicki1998review,rey2015past} for a more detailed overview of this problem. Traditional spike sorting approaches \cite{quiroga2004unsupervised,chung2017fully,yger2018spike,chaure2018novel} are often time consuming, lacking standardization, and involving manual intervention, which makes it difficult to maintain data provenance and assess the quality of scientific results. 

In the following, we introduce a fully automated approach based on SaS-CDL and nonconvex optimization \cite{song2018spike}. Mathematically, the spike sorting problem can be modeled as a superposition of several convolutions of neuron waveform templates and spike trains,
\begin{align*}
   \underbrace{\mb y}_{\text{voltage signal}} \quad = \quad \sum_{k=1}^N \quad \underbrace{ \mb a_{0k} }_{\text{waveform template} } \conv \quad \underbrace{ \mb x_{0k} }_{\text{sparse spike train}} \quad  + \underbrace{\quad b \mb 1_m}_{\text{bias}}  \quad +\quad \underbrace{ \mb n }_{\text{noise}},
\end{align*}
where the waveform templates $\Brac{\mb a_{0k}}_{k=1}^N \in \bb R^{\di}$ for different types of neurons exhibit different kernel shapes. Therefore, Given the signal $\mb y$, the task of spike sorting is to recover all $\Brac{\mb a_{0k}}_{k=1}^N$ and $\Brac{\mb x_{0k}}_{k=1}^N$. This can be naturally cast as a SaS-CDL problem as we discussed in Section \ref{subsec:cdl}.

The difficulty of spike sorting (or SaS-CDL) is not only captured by the self shift-incoherence of each individual waveforms $\mb a_{0k}$, but is also characterized by the shift ''dissimilarity'' between different waveforms $\Brac{ \mb a_{0k} }_{k=1}^N$. The problem becomes increasing more difficult when all the kernels become more similar (i.e., more correlated). Let $\mb A_0 = \begin{bmatrix}
 \mb a_{01} & \cdots & \mb a_{0N}	\end{bmatrix}$. Quantitatively, we can define \emph{mutual incoherence} of $\mb A_0$ by
\begin{align*}
   \mu_m\paren{ \mb A_0 } = \max_{ 1\leq i <j \leq N} \norm{ \mb C_{\mb a_{0i}}^* \mb a_{0j} }{ \infty },
\end{align*}
which is essentially the largest shift-correlation between all kernels. The SaS-CDL problem becomes easy when $\mu_m\paren{ \mb A_0 }$ is small, and vice versa. In the following, we demonstrate the effectiveness of the proposed methods for spike sorting on one easy dataset (with small $\mu_m\paren{ \mb A_0 }$) and one difficult dataset (with large $\mu_m\paren{ \mb A_0 }$). 

We demonstrate the proposed reweighting variant of iADM algorithm on a classical spike-sorting dataset\footnote{It can be downloaded online at \url{https://vis.caltech.edu/~rodri/Wave_clus/Wave_clus_home.htm}.}. The signal is sampled at a frequency of $f = 24kHz$, and each time sequence records spiking activities of 3 different types of neurons. The waveform templates are constructed using a database of $594$ different average spike shapes compiled from recordings in the neocortex and basal ganglia. A more detailed description of dataset can be found in Section 4 of \cite{quiroga2004unsupervised}. We test the proposed method on two signal sequences of length $\sample = 10^5$, each measures the spiking activities of three different types of neurons with length $\di = 72$: one signal sequence is easy to deconvolve with low mutual coherence $\mu_m\paren{ \mb A_0 }$, and another is relatively more difficult with larger $\mu_m\paren{ \mb A_0 }$. The data is contaminated by random noise, with noise level $0.05$ (i.e., the standard deviation relative to the amplitude of the spike classes). The recovered waveform and sparse spike train for the ``easy'' case are shown in \Cref{fig:waveform-easy} and \Cref{fig:spiketrain-easy}, respectively. And the results for the ``difficult'' case are shown in \Cref{fig:waveform-easy} and \Cref{fig:spiketrain-easy}. As we observe, the proposed method successfully recovers the waveform templates and spiking locations for each type of neuron. As the latter ``difficult'' signal sequence contains neuron waveform of similar shapes, we observe slightly more false alarms in spike detection.


\begin{figure*}[!htbp]
\centering
%\captionsetup{font=normalsize,labelfont={bf,sf}}
\captionsetup[sub]{font=normalsize ,labelfont={bf,sf}}
\centering
\begin{minipage}[c]{0.32\textwidth}
\subcaption{Neuron 1}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/easy_waveform_neuron_1_005.png}
\end{minipage}
\begin{minipage}[c]{0.32\textwidth}
\subcaption{Neuron 2}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/easy_waveform_neuron_2_005.png}
\end{minipage}
\begin{minipage}[c]{0.32\textwidth}
\subcaption{Neuron 3}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/easy_waveform_neuron_3_005.png}
\end{minipage}
\caption{\textbf{Recovered neuron waveform template of ``easy'' dataset.} The data contains three neurons of \emph{distinct} waveforms, with noise level $0.05$. Each subfigure corresponds to the recovered waveform template of one specific type of neuron.}
\label{fig:waveform-easy}
\end{figure*}


\begin{figure*}[!htbp]
\centering
%\captionsetup{font=normalsize,labelfont={bf,sf}}
\captionsetup[sub]{font=small,labelfont={bf,sf}}
\begin{minipage}[c]{\textwidth}
\subcaption{raw data vs. estimated sequence}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/easy_spiketrain_sequence_005.png}
\end{minipage}
\begin{minipage}[c]{\textwidth}
\subcaption{spike train for Neuron 1}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/easy_spiketrain_neuron_1_005.png}
\end{minipage}
\begin{minipage}[c]{\textwidth}
\subcaption{spike train for Neuron 2}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/easy_spiketrain_neuron_2_005.png}
\end{minipage}
\begin{minipage}[c]{\textwidth}
\subcaption{spike train for Neuron 3}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/easy_spiketrain_neuron_3_005.png}
\end{minipage}
\caption{\textbf{Detected spike train of ``easy'' dataset.} The data contains three neurons of \emph{distinct} waveforms, with noise level $0.05$. The first subfigure shows the estimation of the raw data sequence. The second to fourth subfigures show the predicted spike train for each neuron, respectively.}
\label{fig:spiketrain-easy}
\end{figure*}


\begin{figure*}[!htbp]
%\captionsetup{font=normalsize,labelfont={bf,sf}}
\captionsetup[sub]{font=normalsize ,labelfont={bf,sf}}
\centering
\begin{minipage}[c]{0.32\textwidth}
\subcaption{Neuron 1}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/difficult_waveform_neuron_1_005.png}
\end{minipage}
\begin{minipage}[c]{0.32\textwidth}
\subcaption{Neuron 2}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/difficult_waveform_neuron_2_005.png}
\end{minipage}
\begin{minipage}[c]{0.32\textwidth}
\subcaption{Neuron 3}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/difficult_waveform_neuron_3_005.png}
\end{minipage}
\caption{\textbf{Recovered neuron waveform template of ``difficult'' dataset.} The data contains three neurons of \emph{similar} waveforms, with noise level $0.05$. Each subfigure corresponds to the recovered waveform template of one specific type of neuron.}
\label{fig:waveform-difficult}
\end{figure*}


\begin{figure*}[!htbp]
\centering
%\captionsetup{font=normalsize,labelfont={bf,sf}}
\captionsetup[sub]{font=small,labelfont={bf,sf}}
\begin{minipage}[c]{\textwidth}
\subcaption{raw data vs. estimated sequence}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/difficult_spiketrain_sequence_005.png}
\end{minipage}
\begin{minipage}[c]{\textwidth}
\subcaption{spike train for Neuron 1}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/difficult_spiketrain_neuron_1_005.png}
\end{minipage}
\begin{minipage}[c]{\textwidth}
\subcaption{spike train for Neuron 2}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/difficult_spiketrain_neuron_2_005.png}
\end{minipage}
\begin{minipage}[c]{\textwidth}
\subcaption{spike train for Neuron 3}
\centering
	\includegraphics[width = \linewidth]{figs/spike_sorting/difficult_spiketrain_neuron_3_005.png}
\end{minipage}
\caption{\textbf{Detected spike train of ``difficult'' dataset.} The data contains three neurons of \emph{similar} waveforms, with noise level $0.05$. The first subfigure shows the estimation of the raw data sequence. The second to fourth subfigures show the predicted spike train for each neuron, respectively.}
\label{fig:spiketrain-difficult}
\end{figure*}



